New Directions in Cloud Programming

Nearly twenty years after the launch of AWS, it remains difficult for most developers to harness the enormous potential of the cloud. In this paper we lay out an agenda for a new generation of cloud programming research aimed at bringing research ideas to programmers in an evolutionary fashion. Key to our approach is a separation of distributed programs into a PACT of four facets: Program semantics, Availablity, Consistency and Targets of optimization. We propose to migrate developers gradually to PACT programming by lifting familiar code into our more declarative level of abstraction. We then propose a multi-stage compiler that emits human-readable code at each stage that can be hand-tuned by developers seeking more control. Our agenda raises numerous research challenges across multiple areas including language design, query optimization, transactions, distributed consistency, compilers and program synthesis.

==> ex_bloom.tex <==
table :people, [:pid] => [:contacts, :covid, :vaccinated] 
table :vars

# add_person
interface :in, :ap_in, [:rid] => 
                      [:pid, :contacts, :covid, :vaccinated]
people <= ap_in{|a| 
  [a.pid, a.contacts, a.covid, a.vaccinated]
}

# diagnosed
interface :in, :d_in, [:rid] => [:pid]
people <= (d_in*people).pairs(:pid=>:pid){|d,p| 
  [p.pid, p.contacts, to_lbool(true), p.vaccinated]
}

# add_contact to both sides
interface :in, :ac_in, [:rid] => [:from, :to], 
              {:consistency=>:eventual, atomicity=>false}
people <= (ac_in*people).pairs(:from=>:pid) {|a,p| 
  [p.pid, to_lset([a.to]), p.covid, p.vaccinated]
}
people <= (ac_in*people).pairs(:to=>:pid) {|a,p| 
  [p.pid, to_lset([a.from]), p.covid, p.vaccinated]
}

# likelihood
interface :in, :l_in, [:rid] => [:pid]
interface :out, :l_out, [:rid] => [:likelihood]
l_out <= (l_in*people).pairs(:pid=>:pid) {|l,p| 
  [l.rid, covid_xmission_model(p.contacts)]
}

# trace transitive closure of contacts
interface :in, :t_in, [:rid] => [:pid],
              {:consistency=>:linearizable, :atomic=true}
interface :out, :t_out, [:rid, :from, :to]
scratch :tr_in, [:origin]
scratch :tp_pairs, [:origin, :pid] => 
                    [:contacts, :covid, :vaccinated]
scratch :trace, [:origin, :pid]
tp_pairs <= (tr_in*people).pairs(:origin=>:pid){|t,p| 
  [t.origin] + p
}
tp_pairs <= (trace*people).pairs(:pid=>:pid){|t,p| 
  [t.origin] + p
}
trace <= tp_pairs.flat_map{|tp| 
  tp.contacts.reveal().map{|s| [tp.origin, s]}
}
tr_in <= t_in{|t| [t.pid]}
t_out <= (t_in*trace).pairs{|i,o| [i.rid] + o}

# is_connected. implicitly, consistency is :immutable
# due to monotonicity of a true lbool
interface :in, :isc_in, [:rid] => [:from, :to]
interface :out, :isc_out, [:rid] => [:status]
tr_in <= isc_in{|i| [i.from]}
isc_out <= (isc_in*trace).pairs(:from=>:origin,
                                :to=>:pid){|i,t| 
  [i.rid, to_lbool(true)] 
}
\end{bloomlisting}

==> ex_python.tex <==
\begin{pythonlisting}{Simple COVID-19 Tracker App in Python}
from typing import Set
class Person:
  def __init__(self, pid: int, country: str):
    self.pid = pid
    self.contacts = set()
    self.country = country
    self.covid = self.vaccinated = False
people: Set[Person]
vaccine_count: int

def find_person(pid: int):
  matches = filter(lambda p: p.pid == pid, people)
  return next(matches)
def add_person(pid: int, country: str):
  people.add(Person(pid, country))

def add_contact(id1: int, id2: int):
  find_person(id1).contacts.add(find_person(id2))
  find_person(id2).contacts.add(find_person(id1))

from covid_xmission_model import covid_predict
def likelihood(pid: int):
  return covid_predict(find_person(pid))

# transitive closure of contacts
def trace(start_id: int):
  result: set[Person] = set()
  diff: set[Person] = {find_person(start_id)} 
  while len(diff) > 0:
    result.update(diff)
    diff = set().union(*[p.contacts for p in diff]) - result
  return result
\end{pythonlisting}

% def vaccinate(pid: int): # mutation
%   global vaccine_count 
%   find_person(pid).vaccinated = True
%   vaccine_count = vaccine_count - 1

% def case_counts(): # monotonic lattice-valued query
%   return sum(p.covid for p in people)

% def trace(start_id: int, end_id: int = None): # monotonic Query
%   start_p: Person = find_person(start_id)
%   end_p: Person = None
%   if end_id:
%     end_p = find_person(end_id)
%   result: set[Person] = set()
%   delta: set[Person] = {start_p} 
%   while len(delta) > 0:
%     result.update(delta)
%     if end_p in delta:
%       # stop early and return what's been found so far
%       return result
%     delta = set().union(*[p.contacts for p in delta])
%     delta.difference_update(result)
%   return result

% # monotonic threshold test
% def is_connected(id1: int, id2: int):
%   return len(trace(id1, id2)) > 0

==> ex_sql.tex <==
% -- first three functions below are just simple test cases
% CREATE FUNCTION find_person(integer) RETURNS people AS $$
%   DECLARE
%     retval people;
%   BEGIN
%     SELECT * INTO retval FROM people WHERE id = $1;
%     RETURN retval;
%   END;
% $$ LANGUAGE plpgsql;
% CREATE FUNCTION add_contact(integer, integer) 
% RETURNS void AS $$
%   BEGIN
%     UPDATE people SET contacts = contacts || $2
%      WHERE people.id = $1;
%   END;
% $$ LANGUAGE plpgsql;
\begin{sqllisting}{Simple COVID-19 Tracker App in SQL}
CREATE TYPE person AS (pid integer primary key, 
  contacts integer[], covid bool, vaccinated bool);
CREATE TABLE people OF person;

CREATE HANDLER add_person(people) AS
    INSERT INTO people VALUES($1.*);

CREATE HANDLER diagnosed(integer) AS
    UPDATE people SET covid=true WHERE pid = $1;

CREATE HANDLER add_contact(integer, integer) AS
  BEGIN
    UPDATE people SET contacts = contacts || $2
     WHERE people.id = $1;
    UPDATE people SET contacts = contacts || $1
     WHERE people.id = $2;
  END;
WITH EVENTUAL CONSISTENCY, NO ATOMICITY;

-- use case: Covid likelihood score per person (stochastic)
CREATE HANDLER likelihood(integer) RETURNS float AS
    SELECT covid_xmission_model(contacts) FROM people
     WHERE pid = $1$;

-- use case: Transitive contact list (monotone)
CREATE FUNCTION pod(integer) RETURNS TABLE (pid integer) AS
    WITH RECURSIVE closure(pid) AS (
      SELECT $1
    UNION
      SELECT contact1 AS pid
        FROM closure c, 
             (SELECT p.pid, unnest(contacts) 
                FROM people p) AS flat(pid, contact1)
      WHERE c.pid = flat.pid
    )
    SELECT * from closure;
    
CREATE HANDLER trace(integer) RETURNS TABLE (pid integer) AS
    SELECT * FROM pod(pid);
WITH LINEARIZABLE, ATOMIC;

-- use case: Connected pair predicate (threshold read)
CREATE HANDLER is_connected(integer, integer) 
RETURNS lattice<bool>
AS
  BEGIN
    var retval integer;
    SELECT count(*) into retval
      FROM pod@async($1) t
     WHERE t.pid = $2;
  RETURN retval > 0;
  END;

SET AVAILABILITY (3 AZ);
SET SLO(cost < 0.1c, latency < 1s@p99);
\end{sqllisting}

% % CREATE FUNCTION case_counts() RETURNS integer 
% % AS $$
% %   DECLARE
% %     retval integer;
% %   BEGIN
% %     SELECT count(*) into retval
% %       FROM people
% %      WHERE covid = true;
% %   RETURN retval;
% %   END;
% % $$ LANGUAGE plpgsql;

